Search for $\mathrm{GeV}$-scale axion-like particles in PbPb collisions

A search is performed for the production of axion-like particles with masses in the range 3-10 GeV using PbPb collision data recorded by the LHCb experiment, corresponding to an integrated luminosity of $0.228~\mathrm{nb}^{-1}$ and a nucleon-nucleon centre-of-mass energy of $\sqrt{s_{\mathrm{NN}}}=5.02$ TeV. This is the first search for axion-like particles produced exclusively by two photons ($\gamma\gamma\to a\to\gamma\gamma$) in the forward direction. It extends sensitivity to previously unexplored regions of the parameter space, probing axion-like particle masses and couplings down to 3.0 GeV and $3.2\times10^{-4}~\mathrm{GeV}^{-1}$, respectively. This result provides the most stringent limits to date on the production of axion-like particles from exclusive photon-photon fusion processes with masses between 3 and 5 GeV.

==> LHCb/Authorship_LHCb-PAPER-2026-029-arXiv.tex <==
LHCb collaboration:
R. Aaij,
M. Abdelfatah,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin\'en,
T. Ackernley,
A.A. Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
S. Akar,
K. Akiba,
H. Al Saleh,
P. Albicocco,
J. Albrecht,
R. Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
Z. Amos,
L. An,
L. Anderlini,
P. Andreola,
M. Andreotti,
S. Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L. Arnone,
M. Artuso,
E. Aslanides,
R. Ata\'ide Da Silva,
M. Atzeni,
B. Audurier,
J.A. Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
M. Bai,
Z.B. Bai,
V. Balagura,
A. Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H. Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I.R. Barbosa,
W. Barker,
R.J. Barlow,
M. Barnyakov,
S. Baron,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P.B. Battista,
A. Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N.A. Behling,
S. Belin,
A. Bellavista,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
J.L.M. Berkey,
R. Bernet,
A. Bertolin,
L. Bertsch,
F. Betti,
J. Bex,
O. Bezshyyko,
S. Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Bohare,
C. Bolognani,
R.B. Bonacci,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E. Bottalico,
S.A. Bouchiba,
M. Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J.D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
C. Breitfeld,
J. Brodzicka,
J. Brown,
E. Buchanan,
M. Burgos Marcos,
C. Burr,
E. Butera,
C. Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y. Cai,
Y. Cai,
A. Caillet,
R. Calabrese,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J.I. Cambon Bouzas,
P. Campana,
A. Campomagnani,
A.C. Campos,
A.F. Campoverde Quezada,
Y. Cao,
S. Capelli,
M. Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I. Celestino,
S. Cesare,
A.J. Chadwick,
M. Charles,
Ph. Charpentier,
E. Chatzianagnostou,
R. Cheaib,
M. Chefdeville,
C. Chen,
J. Chen,
S. Chen,
Z. Chen,
A. Chen Hu,
M. Cherif,
S. Chernyshenko,
X. Chiotopoulos,
G. Chizhik,
V. Chobanova,
A. Christakakis,
M. Chrzaszcz,
Y. Chu,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
A. Codovini,
C.S. Codovini,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S. Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J. Connaughton,
A. Contu,
N. Cooke,
A. Corallo,
G. Cordova,
C. Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
G.C. Costantino,
C. Cotirlan,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
N. Crepet,
M. Cruz Torres,
M. Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
X. Dai,
J. Dalseno,
C. D'Ambrosio,
G. Darze,
A. Davidson,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
F. De Gregorio,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
A. De Robertis,
E. De Santis,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S. Dekkers,
L. Del Buono,
B. Delaney,
B. Demaire-Lepape,
J. Deng,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
S. Ding,
Y. Ding,
L. Dittmann,
J.F. Diverchy,
A.D. Docheva,
A. Doheny,
C. Dong,
F. Dordei,
J. Dorta Moreno,
A.C. dos Reis,
J. Dos Santos Oliveira,
A.D. Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M.M. Duras,
J.M. Durham,
O.D. Durmus,
K. Duwe,
A. Dziurda,
S. Easo,
E. Eckstein,
U. Egede,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D. Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
T. Evans,
F. Fabiano,
S. Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K. Farmer,
F. Fassin,
D. Fazzini,
L. Felkowski,
C. Feng,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
B. Fernandez Rodino,
J. Fernandez-John,
A.D. Fernez,
F. Ferrari,
R.F. Ferreira Leite Considera,
F. Ferreira Rodrigues,
R.A. Fini,
R. Fiorenza,
M. Fiorini,
M. Firlej,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A. Fomin,
M. Fontana,
M. Fontes Vaz,
L.A. Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Y. Fu,
Q. F\"uhring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B. Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc\'ia Pardi\~nas,
P. Gardner,
L. Garrido,
C. Gaspar,
A. Gavrikov,
J. George,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F.I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent\`u,
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G\"obel,
L. Golinka-Bezshyyko,
E. Golobardes,
A. Golutvin,
S. Gomez Fernandez,
A.G. Gomez Mongui,
W. Gomulka,
F. Goncalves Abrantes,
I. Gon\c{c}ales Vaz,
M. Goncerz,
G. Gong,
S. Gong,
J.A. Gooding,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
R. Grande Quartieri,
E. Graug\'es,
E. Graverini,
L. Grazette,
G. Graziani,
A.T. Grecu,
N.A. Grieser,
L. Grillo,
C. Gu,
M. Guarise,
L. Guerry,
A.-K. Guseinov,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S. Haken,
G. Hallett,
P.M. Hamilton,
Q. Han,
S. Han,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
T.J. Harris,
L. Hartman,
M. Hartmann,
S. Hashmi,
J. He,
N. Heatley,
A. Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
A. Henrot,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
D. Hutchcroft,
M. Idzik,
P. Ilten,
A. Iohner,
S. Jacevicius,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
A. Jawahery,
C. Jayaweera,
A. Jelavic,
V. Jevtic,
Z. Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y.J. Jiang,
E. Jimenez Moya,
N. Jindal,
M. John,
A. John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J. Juan Castella,
N. Jurik,
I. Juszczak,
K. Kalecinska,
D. Kaminaris,
S. Kandybei,
M. Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
S. Kholodenko,
V. Kholoimov,
G. Khreich,
F. Kiraz,
T. Kirn,
V.S. Kirsebom,
N. Kleijne,
A. Kleimenova,
D. Klekots,
K. Klimaszewski,
M.R. Kmiec,
T. Knospe,
R. Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kooij,
P. Kopciewicz,
P. Koppenburg,
A. Korchin,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E. Kowalczyk,
O. Kravcov,
M. Kreps,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
A. Kupsc,
A. Kurzina,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I. Kyryllin,
D. Lacarrere,
P. Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H. Lee,
R. Lef\`evre,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E.D. Lesser,
B. Leverington,
A. Li,
C. Li,
C. Li,
H. Li,
J. Li,
K. Li,
L. Li,
L. Li,
P. Li,
P.-R. Li,
Q. Li,
T. Li,
T. Li,
W. Li,
Y. Li,
Y. Li,
Y. Li,
Z. Li,
Z. Lian,
Q. Liang,
X. Liang,
Z. Liang,
S. Libralon,
A. Lightbody,
J. Lin,
S. Lin,
T. Lin,
R. Lindner,
H. Linton,
R. Litvinov,
D. Liu,
F.L. Liu,
G. Liu,
K. Liu,
S. Liu,
W. Liu,
X. Liu,
Y. Liu,
Y. Liu,
Y.L. Liu,
G. Loachamin Ordonez,
I. Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F.C.L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C. Lopez Iribarnegaray,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
M. Lupberger,
E. Luppi,
K. Lynch,
J. Lyu,
S. Lyu,
X.-R. Lyu,
H. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. Mack,
I. Mackay,
L.M. Mackey,
L.R. Madhan Mohan,
M.J. Madurai,
D. Magdalinski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
G. Manca,
C. Mancuso,
R. Manera Escalero,
A. Mangalasseri,
F. Manganella,
R. Mangrulkar,
D. Manuzzi,
S. Mao,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
L. Mareso,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L. Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
C. Martinez,
A. Martinez Armas,
D. Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A. Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
C. Matteuzzi,
K.R. Mattioli,
L. Matzner,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D. Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
S.E.R. Medaer,
D. Melnychuk,
D. Mendoza Granada,
P. Menendez Valdes Perez,
F.M. Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
S. Mico,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
B. Mitreska,
D.S. Mitzel,
R. Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E.F. Molina Cardenas,
T. Momb\"acher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A. Moro,
J. Moron,
W. Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. Mu,
N. Muangkod,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M\"uller,
F. Mu\~noz-Rojas,
V. Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
G. Napoletano,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
J. Nicolini,
D. Nicotra,
E.M. Niel,
L. Nisi,
Q. Niu,
B.K. Njoki,
P. Nogarolli,
P. Nogga,
J. Nombela Royo,
C. Normand,
A. Novo Cal,
J. Novoa Fernandez,
G. Nowak,
H.N. Nur,
A. Oblakowska-Mucha,
T. Oeser,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E. Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A. Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L. Palini,
L. Palombini,
M. Palutan,
C. Pan,
X. Pan,
S. Panebianco,
S. Paniskaki,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D. Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A. Paul,
C.J. Pawley,
A. Pellegrino,
J. Peng,
X. Peng,
M. Pepe Altarelli,
S. Perazzini,
H. Pereira Da Costa,
M. Pereira Martinez,
A. Pereiro Castro,
C. Perez,
A. Perez Casas,
P. Perret,
A. Perrevoort,
A. Perro,
M.J. Peters,
A. Petkovic,
K. Petridis,
A. Petrolini,
S. Pezzulo,
J.P. Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L. Piccolo,
B. Pietrzyk,
R.N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V.M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A. Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
B. Rachwal,
R. Racz,
J.H. Rademacker,
M. Rama,
M. Ram\'irez Garc\'ia,
V. Ramos De Oliveira,
M. Ramos Pernas,
G. Ramsey,
M.S. Rangel,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M. Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F. Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
A. Romano,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
W. Rose,
M. Rotondo,
M.S. Rudolph,
G. Ruggiero,
M. Ruiz Diaz,
J. Ruiz Vidal,
J. Ruz Armendariz,
J.J. Saavedra-Arias,
J.J. Saborido Silva,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
H. Schumacher,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G. Scriven,
I. Segal,
S. Sellam,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
B. Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
R.S. Sharma,
L. Shchutska,
T. Shears,
S. Shelton,
J. Shen,
Z. Shen,
S. Sheng,
B. Shi,
J. Shi,
Q. Shi,
W.S. Shi,
E. Shmanin,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
K. Solovieva,
N.S. Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y.S. Song,
F.L. Souza De Almeida,
G. Souza De Castro,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M. Stefaniak,
O. Steinkamp,
F. Suljik,
J. Sun,
L. Sun,
M. Sun,
D. Sundfeld,
P. Svihra,
V. Svintozelskyi,
J. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y.T. Tang,
M.D. Tat,
J.A. Teijeiro Jimenez,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A.R. Thomson-Strong,
R. Thornton,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T.T. Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Torlai,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
A. Upadhyay,
B. Urbach,
A. Usachov,
U. Uwer,
V. Vagnoni,
A. Vaitkevicius,
A. Valassi,
V. Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
P. Varrella,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V\'azquez Sierra,
S. Vecchi,
J. Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D. Vico Benet,
P. Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
N. Walter,
E.J. Walton,
G. Wan,
A. Wang,
B. Wang,
C. Wang,
C. Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N.W. Wang,
X. Wang,
X. Wang,
X. Wang,
X.W. Wang,
Y. Wang,
Y. Wang,
Y. Wang,
Y.H. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z. Weida,
J. Wendel,
B.D.C. Westhenry,
A.S. White,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M.A. Wiegertjes,
C. Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.J. Williams,
M.R.J. Williams,
R. Williams,
S. Williams,
Z. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E. Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
T. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T.X. Xing,
A. Xu,
L. Xu,
M. Xu,
R. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S. Yadav,
K. Yang,
X. Yang,
Y. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
H. Yeung,
H. Yin,
X. Yin,
C.Y. Yu,
J. Yu,
K. Yu,
X. Yuan,
Y Yuan,
S. Zalambani,
J.A. Zamora Saa,
F. Zangari,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C. Zeng,
M. Zeng,
S.H Zeng,
C. Zhang,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
Q.Z. Zhang,
R. Zhang,
S. Zhang,
S.L. Zhang,
Y. Zhang,
Z. Zhang,
J. Zhao,
M. Zhao,
Y. Zhao,
A. Zhelezov,
S.Z. Zheng,
X.Z. Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
V. Zhovkovska,
L.Z. Zhu,
X. Zhu,
X. Zhu,
Y. Zhu,
V. Zhukov,
J. Zhuo Gao,
T. Zies,
D. Zuliani,
X. Zuo

==> LHCb/Authorship_LHCb-PAPER-2026-029_acknowledgements.tex <==
% Individual acknowledgements
% Data extracted on September 24th, 2026 at 10:58pm for paper reference LHCb-PAPER-2026-029
\section*{Acknowledgements}

\noindent We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We acknowledge support from CERN and from the national agencies:
ARC (Australia);
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMFTR, DFG and MPG (Germany);
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MCID/IFA (Romania); 
%MSHE (Russia); 
MICIU and AEI (Spain);
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We acknowledge the computing resources that are provided by ARDC (Australia), 
CBPF (Brazil),
CERN, 
IHEP and LZU (China),
IN2P3 (France), 
KIT and DESY (Germany), 
INFN (Italy), 
SURF (Netherlands),
Polish WLCG (Poland),
IFIN-HH (Romania), 
%RRCKI and Yandex LLC (Russia), 
PIC (Spain), CSCS (Switzerland), 
and GridPP (United Kingdom).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We are indebted to the communities behind the multiple open-source
software packages on which we depend.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Individual groups or members have received support from
Australian Government Research Training Program (https://doi.org/10.82133/C42F-K220) (Australia);
UK Research and Innovation (http://dx.doi.org/10.13039/100014013) and Science and Technology Facilities Council  (http://dx.doi.org/10.13039/501100000271) (United Kingdom);
InTalent-Inditex  (Spain);
Schweizerischer Nationalfonds zur F\&quot;orderung der Wissenschaftlichen Forschung (http://dx.doi.org/10.13039/501100001711) (Switzerland);
Agence Nationale de la Recherche (http://dx.doi.org/10.13039/501100001665) (France).

==> LHCb/Authorship_LHCb-PAPER-20YY-nnn.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' LHCbInternal/main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && sh LHCbInternal/wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard Figures/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) LHCbInternal/$(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm -f LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

